Inverse Optimization: Theory and Applications

Inverse optimization describes a process that is the "reverse" of traditional mathematical optimization. Unlike traditional optimization, which seeks to compute optimal decisions given an objective and constraints, inverse optimization takes decisions as input and determines an objective and/or constraints that render these decisions approximately or exactly optimal. In recent years, there has been an explosion of interest in the mathematics and applications of inverse optimization. This paper provides a comprehensive review of both the methodological and application-oriented literature in inverse optimization.

==> Algorithms/CP_algorithm.tex <==
\begin{algorithm}[t]
\setstretch{1.2}
\caption{A cutting plane algorithm for inverse mixed integer linear optimization}
\label{algo:CP}
\vspace{0.3cm}
\textbf{Input:} Forward optimization model $\FOPMIP(\btheta), \btheta \in \bTheta$; Decision $\bhx$; Prior $\hat\btheta$ \\
\textbf{Output:} Inverse optimization parameter estimate $\btheta^*$
\begin{algorithmic}[1]
%
\State Initialize $\tilde{\set{X}} = \emptyset$; $\tilde\btheta = \hat\btheta$
\State Solve $\FOPMIP(\tilde\btheta)$ and let $\tilde\bx$ be an optimal solution
%
\While{$\tilde\btheta^\tpose \tilde\bx < \tilde\btheta^\tpose \bhx$}
%
\State Update $\tilde{\set{X}} \gets \tilde{\set{X}} \cup \{ \tilde\bx \}$
\State Solve
%
\begin{align*}
    \min_{\btheta} \left\{ \norm{\btheta - \bhtheta}_p \;\Big|\; \btheta^\tpose \bhx \geq \btheta^\tpose \tilde \bx , \; \forall \tilde\bx \in \tilde{\set{X}}, \; \btheta \in \bTheta \right\}
\end{align*}
%
and let $\tilde\btheta$ be an optimal solution
\State Solve $\FOPMIP(\tilde\btheta)$ and let $\tilde\bx$ be an optimal solution
%\State 
\EndWhile \\
\Return $\btheta^* = \tilde\btheta$ %$\bc^* = \bhc^i$
%
%\State Initialization: $i=1$, $\tilde\mX^0 = \{ \hat\bx \}$.
%\State Initialize $i=0, \, \tilde\mX^i = \emptyset, \, \tilde\btheta^i = \hat\btheta$ %\iz{Change font} 
%\State Solve $\FOPMIP(\tilde\btheta^i)$, let $\tilde\bx^{i}$ be its output
%\State $\tilde\mX^i = \{\tilde\bx^i$\}
%\State $\tilde\mX^1 \gets \{\bhx, \tilde\bx^1$\}.
%\While{$(\tilde\btheta^i)^\top(\tilde\bx^i - \bhx) \neq 0$}
%\textbf{Master Problem}: 
%\State $i \gets i+1$
%\State $\tilde\mX^{i} \gets \tilde\mX^{i-1} \cup \{\tilde\bx^{i-1}\}$
%\State Solve $\IOPp(\bhx, \hat\btheta  ; \tilde\mX^{i})$, let $\tilde\btheta^i$ be its optimal solution \label{step:candidate_cost}
%\Comment return candidate cost vector
%\State Solve $\FOPMIP(\tilde\btheta^i)$, let $\tilde\bx^{i}$ be its output
%\Comment a new cut is found
%\EndWhile \\
%\Return $\btheta^* = \tilde\btheta^i$ %$\bc^* = \bhc^i$
\end{algorithmic}
\end{algorithm}

==> Algorithms/IOPd_enumeration.tex <==
\begin{algorithm}[t]
\setstretch{1.2}
\caption{Enumerative algorithm for $\IOPd(\ell_\mathrm{D}, \dataset)$ when $f(\bx, \btheta)$ is not strictly continuous}
\label{algo:IOPd_enumerative_algo}
\vspace{0.3cm}
\textbf{Input:} Forward model $\FOP(\btheta), \btheta \in \bTheta$; Data set $\{(\bhx_i, \FOP_i(\btheta))\}_{i=1}^N$; Resolution $\delta > 0$ \\
\textbf{Output:} Inverse optimization parameter estimate $\btheta^*$
\begin{algorithmic}[1]
%
\State Initialize $\delta$-net $\set{N}(\delta) \subset \bTheta$ that satisfies $\max_{\btheta \in \bTheta} \min_{\bhtheta \in \set{N}(\delta)} \| \btheta - \bhtheta \| \leq \delta$
\For{$\bhtheta \in \set{N}(\delta)$}
\State Compute $L_{\mathrm{D}, \epsilon}(\bhtheta) := $ the optimal value for problem~\eqref{eq:inverse_risk_minimization_epsilon} for fixed $\btheta=\bhtheta$.
\EndFor \\
\Return $\btheta^* \gets \argmin_{\bhtheta \in \set{N}(\delta)} L_{\mathrm{D}, \epsilon}(\bhtheta)$
%\Return $\btheta^* \gets \argmin_{\bhtheta \in \set{N}(\delta)} \{ L_{\mathrm{D}, \epsilon}(\bhtheta) \;|\; \bhtheta \in \set{N}(\delta) \}$
%
%\State Initialization: $i=1$, $\tilde\mX^0 = \{ \hat\bx \}$.
%\State Initialize $i=0, \, \tilde\mX^i = \emptyset, \, \tilde\btheta^i = \hat\btheta$ %\iz{Change font} 
%\State Solve $\FOPMIP(\tilde\btheta^i)$, let $\tilde\bx^{i}$ be its output
%\State $\tilde\mX^i = \{\tilde\bx^i$\}
%\State $\tilde\mX^1 \gets \{\bhx, \tilde\bx^1$\}.
%\While{$(\tilde\btheta^i)^\top(\tilde\bx^i - \bhx) \neq 0$}
%\textbf{Master Problem}: 
%\State $i \gets i+1$
%\State $\tilde\mX^{i} \gets \tilde\mX^{i-1} \cup \{\tilde\bx^{i-1}\}$
%\State Solve $\IOPp(\bhx, \hat\btheta  ; \tilde\mX^{i})$, let $\tilde\btheta^i$ be its optimal solution \label{step:candidate_cost}
%\Comment return candidate cost vector
%\State Solve $\FOPMIP(\tilde\btheta^i)$, let $\tilde\bx^{i}$ be its output
%\Comment a new cut is found
%\EndWhile \\
%\Return $\btheta^* = \tilde\btheta^i$ %$\bc^* = \bhc^i$
\end{algorithmic}
\end{algorithm}
